Single-electron current sources: towards a refined definition of ampere

Controlling electrons at the level of elementary charge $e$ has been demonstrated experimentally already in the 1980's. Ever since, producing an electrical current $ef$, or its integer multiple, at a drive frequency $f$ has been in a focus of research for metrological purposes. In this review we first discuss the generic physical phenomena and technical constraints that influence charge transport. We then present the broad variety of proposed realizations. Some of them have already proven experimentally to nearly fulfill the demanding needs, in terms of transfer errors and transfer rate, of quantum metrology of electrical quantities, whereas some others are currently "just" wild ideas, still often potentially competitive if technical constraints can be lifted. We also discuss the important issues of read-out of single-electron events and potential error correction schemes based on them. Finally, we give an account of the status of single-electron current sources in the bigger framework of electric quantum standards and of the future international SI system of units, and briefly discuss the applications and uses of single-electron devices outside the metrological context.

==> rmp_ch3_8_VM.tex <==
\subsection{Reaching the metrological level of accuracy and current magnitude in hybrid structures}
The obtainable accuracy of a single-electron source is of prime interest especially for metrological applications. In this section we consider two main effects which limit the accuracy, namely the higher order tunneling processes and the relaxation of quasiparticle excitations. When higher order tunneling takes place, more than one electron tunnel simultaneously instead of the wanted single electon. The extra electrons leaking through cause excessively high current. The other leakage process arises as transfered electrons create excitations. These excitations lying at high energy states can then easily tunnel again and cause errors unless the relaxation of the electrons is made strong enough. It turns out to be crucial to take care of the relaxation as seen in the following sections.

In addition to the accuracy of the pumped current, the output signal should be large enough to make measurements in reasonable averaging time. We will address the obtainable output current level and possibility of parallelization in the last part of the section.

\subsubsection{Higher order tunneling processes}
As discussed in sections~\ref{todo}~-~\ref{todo}, the operation of single electron pumps is based on sequential tunneling of electrons which is disturbed by simultaneous tunneling of several electrons. For fully normal metallic pumps, the most important process is co-tunneling where multiple electrons tunnel through Coulomb blockaded islands without suffering any energy cost related to charging. This leads to leakage current proportional to $R_T^{-N}$, where $N$ is the number of tunneling events needed to avoid charge ending up to a Coulomb blockaded islands and $R_T$ is the tunneling resistance of one junction~\cite{Jensen1992}. To obtain the accuracy requirements for metrological applications, one needs to make a chain of islands leading to slower operation speed and more complex control~\cite{Martinis1994,Keller1996,Keller1999}.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/andreevPumping}
	\caption{\label{fig:andreevPumping} (a) Stability diamonds for single-electron tunneling (blue solid lines) and Andreev tunneling (red dotted lines) for sample with $E_c > \Delta$. (b) Stability diamonds for sample with $E_c < \Delta$. (c) First pumping plateau of the high $E_c$ device as a function of the gate voltage amplitude $A_g$. The solid symbols show pumped current with $f= 10\ \mathrm{MHz}$ and three different bias voltages. Dotted lines are the simulated traces with the corresponding biasing. (d) The same data as in (c) but now for the low $E_c$ device showing excess current due to Andreev tunneling.}
\end{figure}

For the hybrid structures where tunneling takes place between a superconductor and a normal metal, co-tunneling is avoided at low biasing. Since there is no available states in the superconductor inside the gap, co-tunneling starts only after biasing each of the junctions by a voltage $V \geq \Delta/e$. This reflects the fact that one needs to provide energy greater or equal to $\Delta$ for each tunneled electron which breaks a Cooper pair. The pumping operation is obtained with voltages well below this threshold and hence co-tunneling is suppressed. 

For hybrid structures, the lowest order tunneling process, where the energy cost of breaking a Cooper-pair can be avoided, is Andreev tunneling~\cite{Andreev1964}, where a complete Cooper-pair tunnels through a junction. Andreev tunneling has been studied thoroughly with single NIS junctions~\cite{Blonder1982,Eiles1993,Lafarge1993,Hekking1994,Pothier1994,Rajauria2008,Greibe2011,Maisi2011} as well as in so-called Cooper-pair splitters where the electrons of a Cooper pair tunnel to different normal metal regions~\cite{Hofstetter2009,Wei2010,Herrmann2010}. In the case of a SINIS turnstile, the Andreev tunneling takes place so that either two electrons are added to or removed from the central island. This implies that when the charging energy of the device is increased, the energy cost\footnote{todo: Thresholds should be discussed here if not done in previous sections.} for charging the island becomes higher and therefore Andreev tunneling becomes suppressed as well~\cite{Averin2008,Maisi2011}. The effect of Andreev tunneling to the accuracy of a turnstile has been directly observed on the pumped current~\cite{Aref2011}. In Fig.~\ref{fig:andreevPumping} stability diamonds for single electron and Andreev tunneling are shown for high $E_c$ device (a) and low $E_c$ device (b). The pumping plateau of high $E_c$ device, shown in (c), is free of Andreev tunneling whereas the low $E_c$ sample exhibits it as seen in (d).

For high charging energy devices, as Andreev tunneling is suppressed, the process limiting the accuracy of the SINIS turnstile will be co-tunneling of a Cooper pair and a single electron~\cite{Averin2008}. In this process, the island will be charged or discharged by a single electron as in one-electron process but in addition, effectively, another electron passes the device. Therefore the energy gain for this process is always at least as high as for one-electron process and the process cannot be suppressed by tuning the device parameter values. By making the junctions opaque enough, the error will be sufficiently low. Ideally, to obtain relative accuracy of $\delta I/I = 10^{-7}$, one needs to limit the speed of a turnstile to a few tens of $\mathrm{pA}$. The operation is expected to slow down by an additional factor of $3$ since the tunnel barriers are not uniform~\cite{Maisi2011,Aref2011}.

\subsubsection{Quasiparticle relaxation}

Single electron tunneling to or from a superconductor will generate quasiparticle excitations. Let us now consider the error caused by these excitations. The quasiparticles relax quickly internally, so that at low temperatures we can assume them to lie close to the gap edges and have a temperature $T_{qp}$ which is higher than the bath temperature of the system. With this assumption, we can calculate the density of the quasiparticle excitations to be
\begin{equation}
\label{eq:nqp}
\begin{array}{rcl}
n_{qp} & = & 2 D(E_F) \displaystyle\int_\Delta^\infty dE n_S(E) e^{-\beta E}\\
            & = &  \displaystyle\sqrt{2 \pi}D(E_F)\Delta\frac{e^{-\beta\Delta}}{\sqrt{\beta\Delta}},
\end{array}
\end{equation}
where we have assumed $e^{-\beta\Delta} \ll 1$ and that the branch imbalance is negligible. The tunneling rate caused by the excitations can be calculated from Eq.~(\ref{todo}) and depends linearly on the density and is independent on biasing at low energies: $\Gamma_{qp} = n_{qp}/(2 e^2 R_T D(E_F))$. Now we should compare this rate causing the errors to the rate at which we pump electrons. The pumping speed of a turnstile is limited approximately to $f = \Delta/(10 e^2 R_T)$, where we have assumed that one needs $5$ time constants for each tunneling of a single electron. To obtain relative accuracy of $\delta I/I$, we must have $\Gamma_{qp} < (\delta I/I) f$ leading to condition $n_{qp} < \frac{1}{5} D(E_F) \Delta \cdot \delta I /I$. With parameter values $D(E_F) = 1.45 \cdot 10^{47}\ \mathrm{J^{-1}m^{-3}}$ and $\Delta = 200\ \mathrm{\mu eV}$, typical to aluminum, and with the asserted accuracy level $\delta I/I = 10^{-7}$, we need $n_{qp} < 0.1\ \mathrm{\mu m^{-3}}$. Such a low level is demonstrated in an experiment without active driving of the system~\cite{Saira2012}, and is sensitive to the filtering and shielding of the sample. Also the trapping of quasiparticles is shown to cruicial in that set of experiments.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/relaxation}
	\caption{\label{fig:relaxation} Two most typical geometries for a superconducting bias lines: (a) A line with constant cross-section determined by the thickness $d$ and width $w$. The lenght of the line is $l$. (b) A line which opens up starting from radius $r_0$ and ending at $r_t$. For the picture the opening angle $\theta$ is set to $\theta = 180^\circ$. The brown parts on top denote the possible place for a quasiparticle trap. Panel (c) presents quasiparticle density $n_{qp}$ along a constant cross section line with various oxide trap transparencies $k$ and panel (d) along an opening line. $n_{qp}$ is scaled with respect to $n_i = Dl P_{inj}/A_i$, where injenction area $A_i = wd$ for panel (c) and $A_i = \theta r_0 d$ for panel (d). For the opening line we also use notation $x = (r-r_0)/l$ with $l = r_t - r_0$ and have used values $r_0 = 20\ \mathrm{nm}$ and $r_t = 5\ \mathrm{\mu m}$.}
\end{figure}

 Next, we need to consider the relaxation of the quasiparticles. When the electrons are being pumped, they are actively driven out of equilibrium. We model the quasiparticle relaxation by heat diffusion in a superconductor and obtain a diffusion equation for $n_{qp}$. Such an approach has been used to model several experiments~\cite{Rajauria2009-2,Ullom1998,Oneil2011,Peltonen2011}. The heat flow of quasiparticles $\vec{J}$ follows the equation $\nabla \cdot \vec{J} = -p$, where $p$ is the power per unit volume removed from the quasiparticles. We use Fourier's law of heat conduction: $\vec{J} = - \kappa_S \nabla T$, where $\kappa_S = \frac{6}{\pi^2} \frac{L_0 T}{\rho_n} \left(\beta \Delta \right)^2 e^{-\beta \Delta}$, is the heat conductivity of a superconductor~\cite{Bardeen1959}. Here $L_0$ is Lorenz number and $\rho_n$ the resistivity in normal state. By taking the derivatives only over strong exponential dependencies and using Eq.~(\ref{eq:nqp}) we obtain diffusion equation
\begin{equation}
\label{eq:diff}
D \nabla^2 n_{qp} = p,
\end{equation}
where the coefficient $D = \frac{\sqrt{2}(k_BT\Delta)^{1/2}}{\sqrt{\pi}e^2\rho_n D(E_F)}$ is assumed to be constant. Now we need to consider different relaxation mechanisms of heat. Inherent mechanism for the quasiparticles inside the superconductor is electron-phonon coupling. However, it is so weak that the decay lenght is typically on the millimeter scale~\cite{Martinis2009,Peltonen2011}. Typically, to enhance, the relaxation, one uses so-called quasiparticle traps~\cite{Pekola2000,Rajauria2009-2,Oneil2011}, which are normal metallic regions connected either directly to the superconductor or separated by an oxide layer. The hot quasiparticles transfer to those regions where the stronger relaxation of a normal metal removes the heat. With the direct coupling, we assume that the quasiparticles relax at the interface to the temperature set by the normal metallic region. This sets a boundary condition for Eq.~(\ref{eq:diff}). Another boundary condition is obtained at the junction where the heat flow is set to the injected power of the device. With the oxide trap, the relaxation is caused by the quasiparticle tunneling. From Eq.~(\ref{todo}) we obtain the heat flow through such a trap as
\begin{equation}
\label{eq:relaxTrap}
\begin{array}{rcl}
p & = & \displaystyle\frac{2 \sigma_T}{e^2 d}\int_\Delta^\infty dE E n_S(E)(e^{-\beta E}-e^{-\beta_0 E}) \vspace{5pt} \\
   & = & \displaystyle\frac{\sigma_T}{e^2 D(E_F) d}(n_{qp}-n_{qp0}),
\end{array}
\end{equation}
by setting $\delta E = 0$. Here $\sigma_T$ is the conductance per unit area and $d$ thickness of the superconducting film. $\beta = k_B T$ and $\beta_0 = k_B T_0$, where $T_0$ is the temperature of the normal metal electrons. $n_{qp0}$ is the quasiparticle number at temperature $T_0$, i.e. assuming that the superconductor would be thermalized to the normal metal fully.

Now we are ready to consider typical superconducting lines used in devices. First let us consider a very typical case: a lead with a constant cross-section as shown in Fig.~\ref{fig:relaxation} (a). We assume that heat $P_{inj}$ is injected on one end of the line and the other end is thermally anchored by a direct trap. For the line itself, we take an oxide trap to be located on top and we can solve Eqs.~(\ref{eq:diff}) - (\ref{eq:relaxTrap}) analytically in one dimension to obtain $n_{qp}(x) = \frac{1}{D\sqrt{k}} (e^{\sqrt{k}(2l-x)}-e^{\sqrt{k}x}) (e^{2 \sqrt{k}l}+1)^{-1}\frac{P_{inj}}{wd}+n_{qp0}$. Here $k = \frac{\sqrt{\pi}\rho_n \sigma_T \Delta}{\sqrt{2}(k_BT\Delta)^(1/2) d}$, and $x$ is the coordinate along the wire starting from the injection side ($x=0$) and ending to the direct trap ($x =l$). In Fig.~\ref{fig:relaxation} (c), we show the quasiparticle density for various $\sigma_T$. The lowest $\sigma_T$ corresponds to the case where the quasiparticles only diffuse through the wire and then relax at the direct contact. At larger transparencies, the oxide trap starts to help for the relaxation as well. If we use parameter values, $d = 50\ \mathrm{nm}$, $w = 100\ \mathrm{nm}$, $l = 1\ \mathrm{\mu m}$ and $T = 130\ \mathrm{mK}$ which are typical for fabricated samples, we see that a typical injection power of $P_{inj}= 2\ \mathrm{fW}$ will yield $n_{qp}-n_{qp0} = 10\ \mathrm{\mu m^{-3}}$ without the oxide trap and even with the highest transparency $\sigma_T = (100\ \mathrm{k\Omega \mu m^2})^{-1}$, which is possible to fabricate without pinholes~\cite{Brenning2004}, we get only an order of magnitude improvement.

To decrease the quasiparticle density to the acceptable level discussed in the beginning, one needs to optimize the lead geometry as well. Therefore, let us consider a lead which starts to widen straight from the junction as shown in  Fig.~\ref{fig:relaxation} (b). In this case we can solve one dimensional diffusion equation in polar coordinates. The junction is assumed to be located at radius $r = r_0$ and the direct contact trap to begin at radius $r = r_t$. Thickness of the film is $d$ and on top of it, there's an oxide trap. The solution of Eqs.~(\ref{eq:diff}) - (\ref{eq:relaxTrap}) can be expressed with modified Bessel functions $I_\alpha$ and $K_\alpha$ as $n_{qp}(r) =n_{qp0} + \frac{1}{D\sqrt{k}} \frac{P_{inj}}{\theta r_0 d} \{ (K_1(\sqrt{k}r_0)+\frac{K_0(\sqrt{k}r_t)}{I_0(\sqrt{k}r_t)}I_1(\sqrt{k}r_0))^{-1}K_0(\sqrt{k}r) + (I_1(\sqrt{k}r_0)+\frac{I_0(\sqrt{k}r_t)}{K_0(\sqrt{k}r_t)}K_1(\sqrt{k}r_0))^{-1} I_0(\sqrt{k}r) \}$. In Fig.~\ref{fig:relaxation} (d) we have plotted $n_{qp}(r)$ for various transparencies of the oxide trap. The lowest transparencies again correspond to pure diffusion limit. As can be seen, the quasiparticle density at the junction depends only weakly on the transparency of the trap: Changing the transparency several orders of magnitude, makes less than an order of magnitude difference to $n_{qp}(r_0)$. This reflects the fact that in the widening lead, the heat sinking is made efficient by spreading the heat to a larger volume and then even a weak relaxation rate is sufficient for the final sinking. By using realistic parameter values,  $d = 50\ \mathrm{nm}$, $\theta = \pi/2$, $r_0 = 50\ \mathrm{nm}$, $r_t = 5\ \mathrm{\mu m}$, $T = 130\ \mathrm{mK}$ and $P_{inj}= 2\ \mathrm{fW}$, we see that it is possible to reach $n_{qp} < 1\ \mathrm{\mu m^{-3}}$ at the junction even without an oxide trap. By increasing the thickness of the electrode by a factor of ten would then start to be sufficient for the accuracy requirements.

Several experiments~\cite{Rajauria2009-2,Ullom1998,Oneil2011} show that the above diffusion model is valid for quasiparticle densities of the order of $n_{qp} \sim 10\ \mathrm{\mu m^{-3}}$. The hundred times smaller quasiparticle density required for metrological applications implies that actual number of the quasiparticles becomes very small. With a typical volume of a lead, $100\ \mathrm{nm} \times 100\ \mathrm{\mu m^2}$, the quasiparticle number is $N < 1$ with $n_{qp} < 0.1\ \mathrm{\mu m^{-3}}$. It is not yet know if such a situation can be treated with the diffusion model or whether a more elaborated theory is required. Pumping experiments on metrological accuracy can provide a way to study such a situation.



%Now, let us consider a lead with thickness $d$, widht $w$ and lenght $l$. In the case of no trap ($p = 0$), we obtain $n_{qp}$


%by solving Eq.~(\ref{eq:diff}). $P_{inj}$ is the power injected to the line: $P_{inj} = d w (-\kappa_S \nabla T_{qp})$.

\subsubsection{Parallelization}
With the normal-metal single-electron pump, it is possible to reach precise enough pumping cycle by having sufficiently long array of islands. With six island, seven junction pump, the accuracy of the pumped current is on $\delta I/ I \sim 10^{-7}$ level. However, the maximum current is limited to a few $\mathrm{pA}$  since one needs to wait for each island the wanted tunneling to occur. To get the current on $100\ \mathrm{pA}$ level, a requirement for a practical metrological applications, see Sect.~\ref{todo}, approximately hundred pumps should be operated in parallel. The main reason why paralelization is inpractical for normal-metal devices is the tuning of the offset charges. Each of the island has an individual offset charge which has to be compensated separately. Therefore the parallelization of normal metallic pumps requires thousand gate voltages for the tuning. Also the offset charges tend to drift and jump. Hence all the offsets needs to be checked every now and then.

The complexity of a normal metallic pump can be avoided by using a quantum dot pump. For these pumps it is possible to tune the barrier heights during pumping cycle which allows to close the transport channel when electron transport is not wanted and open it as transport is desired. Therefore it is expected that the pumping speed can be increased without losing in accuracy. It is possible to use a single dot instead of an array which reduces the number of required control signals. With such a pump, $15\ \mathrm{ppm}$ accuracy at output current of approximately $55\ \mathrm{pA}$ is demonstrated with a single quantum dot~\cite{Giblin2010}. To parallelize a few of those would be then sufficient to reach the required output current level for applications. With two pumps, invariancewith respect to gate variations has been show to be below $20\ \mathrm{ppm}$ level~\cite{Wright2009} with output current exceeding $100\ \mathrm{pA}$. In this case, all signals were individually tuned for each device requiring two dc and one rf signal per device. However, it is possible to use common signals for rf drive and one of the barrier voltages~\cite{Mirovsky2010}. In this case, only one dc voltage per device is required for tuning the other barrier and possible offset charges. The obtainable accuracy, depending on device similarity, is still an open question for this approach.

For the hybrid NIS turnstiles, the maximum current per device is limited to a few tens of picoamperes, as discussed in Sect.~\ref{todo}. Hence, approximately ten devices are needed in parallel, which is experimentally shown to be feasible~\cite{Maisi2009}. However, the pumps in those experiments suffered from environmental activated tunneling errors, so the quantization accuracy was only on $10^{-3}$ level and should be higher for more recent devices~\cite{Pekola2010}. 

For parallelizing the turnstiles, the biasing can be made common since it is determined by the superconducting gap of aluminum, which is a material constant and depends only weakly on the thickness of the Al film. Also, the rf drive can be made common if the devices have similar enough $R_T$, $E_c$ and coupling from the rf gate to the island. The pumping frequency has to be chosen according to the slowest device. Therefore, even if the fastest devices are individually accurate enough, the relative pumping error might become larger as some of the devices have to be operated below the optimal speed. Also the optimal amplitude can vary depending on device parameter values. Depending on which process is limiting the accuracy of a single device, it sets a certain amplitude regime where the current quantization is sufficient. How the regime depends on device parameter values sets then constraints on the device similarity. As the error process limiting the accuracy is not yet determined, the final requirements can not be fully resolved. On the other hand, one can try to make more similar devices by improving the fabrication process. The variation of the critical parameter values depends on the quality of the lithography defining the geometry of the structures and the uniformity of the oxide barrier creating the tunnel junctions.

%-Figure showing 10 parallel devices and parallel QDs.

%-Figure with good pumping plateaus: accuracy limitation on: qp density, 3e process (laborous to do..), back tunneling, i.e. only 1e processes?

%-Paragraph about offset charge stablity and it's effects?
